Majorizing Measures, Sequential Complexities, and Online Learning

We introduce the technique of generic chaining and majorizing measures for controlling sequential Rademacher complexity. We relate majorizing measures to the notion of fractional covering numbers, which we show to be dominated in terms of sequential scale-sensitive dimensions in a horizon-independent way, and, under additional complexity assumptions establish a tight control on worst-case sequential Rademacher complexity in terms of the integral of sequential scale-sensitive dimension. Finally, we establish a tight contraction inequality for worst-case sequential Rademacher complexity. The above constitutes the resolution of a number of outstanding open problems in extending the classical theory of empirical processes to the sequential case, and, in turn, establishes sharp results for online learning.

==> Sections/proof-chaining.tex <==

\section{Proof of Theorem \ref{thm:chaining}}\label{app:chaining}
In order to chain, we need an adaptive tail bound for the tree process.  We have
\begin{lemma}\label{lem:adaptivetail}
	Let $\vbf$ be a labelled binary tree and let $\epsilon_1, \dots, \epsilon_n$ be independent Rademacher random variables.  Then for any $y > 0$, with probability at least $1 - \rho$, we have
	\begin{equation}
		\sum_{t = 1}^n \vbf_t(\epsilon)^2 \leq y
	\end{equation}
	implies that
	\begin{equation}
		\abs{\sum_{t = 1}^n \epsilon_t \vbf_t(\epsilon)} \leq 2\sqrt{2y\log \frac 1\rho}
	\end{equation}
\end{lemma}
\begin{proof}
	Let
	\begin{equation}
		M_s = \sum_{t \leq s} \epsilon_t \vbf_t(\epsilon)
	\end{equation}
	Note that $M_s$ is a martingale with conditionally symmetric increments because the $\epsilon_t$ are independent and the $\vbf_t$ are adapted.  Note that the quadratic variation is given by $[M_s] = \sum_{t = 1}^n \vbf_t(\epsilon)^2$.  Thus by de la Pena's inequality (see \cite{victor1999general,bercu2008exponential}), we have for any $x, y > 0$,
	\begin{equation}
		\pp\left(\abs{M_T} \geq x, \,\, [M_T] \leq y \right) \leq 2e^{- \frac{x^2}{2 y}}
	\end{equation}
	Setting $x = 2 \sqrt{2 y \log \frac 1\rho}$ concludes the proof.
\end{proof}

We are now ready to prove the main chaining bound with the fractional covering number.  For $\vbf,\vbf' \in \mathcal{V}$ binary trees, we fix
\begin{align}
	\mathbb{T}_{\vbf,\vbf'}(\epsilon) = \sum_{t = 1}^n \epsilon_t (\vbf_t(\epsilon) - \vbf_t'(\epsilon))
\end{align}
and we recall that the norm is
\begin{align}
	\norm{\vbf(\epsilon) - \vbf'(\epsilon)} = \sum_{t = 1}^n (\vbf_t(\epsilon) - \vbf_t'(\epsilon))^2
\end{align}
With this notation fixed, we can prove Theorem \ref{thm:chaining}
\begin{proof}
	The second statement follows from the first by integrating the tail bound.  For the first, we note that by monotonicity and linearity of the integral, it suffices to show that with probability at least $1 - \rho$,
	\begin{align}
		\sup_{f \in \mathcal{F}} \mathbb{T}_f(\epsilon) &\leq C \sqrt{n \log \frac 1\rho} + \sqrt n \delta_N  + C\sum_{j = 0}^N  \delta_j\sqrt{\log N'(\mathcal{F}, \delta_j,\z)} \\
		&\leq C \sqrt{n \log \frac 1\rho} + \sqrt n \delta_N + C\sum_{j = 0}^N  \delta_j 2^{\frac j2}
	\end{align}
	where $\delta_j$ is the minimal $\delta > 0$ such that $N'(\mathcal{F}, \delta, \z) \leq 2^{2^j}$.  Henceforth, we fix $\z$ and let $N'(\F, \delta) = N'(\F, \delta, \z)$.  For convenience, let $\gamma_j = 2^{2^j}$ and let $\mu_j$ be a fractional cover of size $N'(\mathcal{F}, \delta_j)$.  By separability, we may approximate $\mathcal{F}$ by a sequence of finite sets and so we may assume that $\mathcal{F}$ is finite.  With high probability on $\epsilon$, for every $f$ we wish to construct a chain $\vbf_{f,j,\epsilon}$ such that $\vbf_{f,j,\epsilon}(\epsilon)$ is close to $f$ and the size of the ``links'' of the chain are small.
	
	We claim that if $j_0 = \lceil \log\log \frac 1\rho \rceil$ then with probability at least $1 - \rho$, the following (which we refer to as \hypertarget{events}{($\ast$)}) hold:
	\begin{align}
		&\mu_{j_0}\left(\left\{\vbf | \abs{\mathbb{T}_\vbf(\epsilon)} > C \sqrt{n \log \frac 1\rho} \right\}\right) \leq \frac 1{3 \gamma_{j_0}}  \\
		&\forall j \geq j_0, \, \nu_j\left(\left\{(\vbf,\vbf') | \abs{\mathbb{T}_{\vbf,\vbf'}(\epsilon)} > C   \delta_j \sqrt{n \log \gamma_j} \text{ and } \norm{\vbf(\epsilon) - \vbf'(\epsilon)} \leq 2 \delta_j\sqrt{n} \right\}\right) \leq \frac{1}{9 \gamma_j \gamma_{j+1}}
	\end{align}
	where $\nu_j = \mu_j \otimes \mu_{j + 1}$ and we recall that
	\begin{equation}
		\mathbb{T}_{\vbf,\vbf'}(\epsilon) = \sum_{t = 1}^n \epsilon_t \left(\vbf_t(\epsilon) - \vbf_t'(\epsilon \right)
	\end{equation}
	The proof of \hyperlink{events}{($\ast$)} is given in Lemma \ref{lem:chainingunionbound} below; for now assume that it is true.  Consider the following sets:
	\begin{align}
		A_j(f, \epsilon) &= \left\{\vbf| \norm{\vbf(\epsilon) - f(\z(\epsilon))} \leq \sqrt n \delta_j \right\} \\
		A_j'(f, \epsilon) &= \left\{\vbf \in A_j(f,\epsilon)| \mu_{j + 1}\left(\left\{\vbf' | \abs{\mathbb{T}_{\vbf,\vbf'}(\epsilon)} > C  \delta_j \sqrt{n \log \gamma_j} \text{ and } \norm{\vbf(\epsilon) - \vbf'(\epsilon)} \leq 2 \delta_j \sqrt{n} \right\}\right) \leq \frac 1{3 \gamma_{j+1}} \right\}
	\end{align}
	By definition of the fractional cover, $\mu_j(A_j(f,\epsilon)) \geq \frac 1{\gamma_j}$.  We lower bound $\mu_j(A_j'(f, \epsilon))$, assuming we have $\epsilon$ such that \hyperlink{events}{($\ast$)} holds.  For any $\vbf$, let
	\begin{equation}
		B(\vbf) = \left\{\vbf' | \abs{\mathbb{T}_{\vbf,\vbf'}(\epsilon)} > C  \delta_j \sqrt{n \log \gamma_j} \text{ and } \norm{\vbf(\epsilon) - \vbf'(\epsilon)} \leq 2 \delta_j \sqrt{n} \right\}
	\end{equation}
	and let
	\begin{equation}
		B = \bigcup_\vbf \bigcup_{\vbf' \in B(\vbf)} \left\{(\vbf,\vbf') \right\}
	\end{equation}
	Let
	\begin{equation}
		\widetilde{B} = \left\{\vbf | \mu_{j + 1}(B(\vbf)) > \frac 1{3 \gamma_{j+1}} \right\}
	\end{equation}
	From \hyperlink{events}{($\ast$)}, we know that $\nu_j(B) \leq \frac 1{9 \gamma_j \gamma_{j+1}}$.  By construction of $\nu_j$, we have
	\begin{align}
		\nu_j(B) = \pp_{\mu_{j +1}}\left(B(\vbf) | \vbf \in \widetilde{B}\right)  \pp_{\mu_j} \left(\widetilde{B}\right)
	\end{align}
	By construction, if $\vbf \in \widetilde{B}$, then
	\begin{equation}
		\pp_{\mu_{j +1}}\left(B(\vbf)\right) \geq \frac 1{3 \gamma_{j+1}}
	\end{equation}
	Thus we have
	\begin{align}
		\pp_{\mu_j} \left(\widetilde{B}\right) = \frac{\nu_j(B)}{\pp_{\mu_{j +1}}\left(B(\vbf) | \vbf \in \widetilde{B}\right) } \leq \frac{\frac 1{9 \gamma_j \gamma_{j+1}}}{\frac 1{3 \gamma_{j+1}}} = \frac 1{3 \gamma_j}
	\end{align}
	Thus we see that
	\begin{equation}
		\mu_j(A_j'(f, \epsilon)) \geq \mu_j(A_j(f, \epsilon)) - \mu_j(\widetilde{B}) \geq \frac 1{\gamma_j} - \frac 1{3 \gamma_j} = \frac 2{3 \gamma_j}
	\end{equation}
	As a final remark before we construct the chain, note that if $\vbf \in A_j(f, \epsilon)$ and $\vbf' \in A_{j+1}(f, \epsilon)$, then by the triangle inequality,
	\begin{equation}\label{eq:triangle}
		\norm{\vbf(\epsilon) - \vbf'(\epsilon)} \leq \norm{\vbf(\epsilon) - f(\z(\epsilon))} + \norm{\vbf'(\epsilon) - f(\z(\epsilon))} \leq \delta_j \sqrt{n} + \delta_{j+1} \sqrt{n} \leq 2 \delta_j \sqrt n
	\end{equation}
	We are now ready to construct the chain.  Fix $\epsilon$ such that \hyperlink{events}{($\ast$)} holds.  For notational simplicity, we suppress the dependence of $\vbf_{f,j,\epsilon}$ on $\epsilon$ and simply write $\vbf_{f,j}$; this causes no confusion as we have fixed $\epsilon$.  For any $f$, we have
	\begin{align}
		\mu_{j_0}\left(A_{j_0}'(f,\epsilon) \cap \left\{\vbf | \abs{\mathbb{T}_\vbf(\epsilon)} > C \sqrt{\n\log \frac 1\rho} \right\}^c\right) \geq \frac 2{3 \gamma_j} - \frac 1{3 \gamma_j} = \frac 1{3\gamma_j} > 0
	\end{align}
	Thus there exists a $\vbf_{f,j_0} \in A_{j_0}'(f,\epsilon)$ such that
	\begin{equation}
		\abs{\mathbb{T}_{\vbf_{f,j_0}}(\epsilon)} \leq C \sqrt{n \log \frac 1\rho}
	\end{equation}
	Now suppose that we have chosen $\vbf_{f,j} \in A_j'(f, \epsilon)$.  We wish to select an element $\vbf_{f, j+1} \in A_{j+1}'(f, \epsilon)$ such that $\abs{\mathbb{T}_{\vbf_{f,j}, \vbf_{f,j+1}}(\epsilon)}$ is small.  To see that this is possible, we remark that, as $\vbf_{f,j} \in A_j'(f, \epsilon)$, we have by definition
	\begin{align}
		\mu_{j + 1}\left(\left\{\vbf' | \abs{\mathbb{T}_{\vbf_{f,j},\vbf'}(\epsilon)} > C \sqrt n \delta_j \sqrt{\log \gamma_j} \text{ and } \norm{\vbf_{f,j}(\epsilon) - \vbf'(\epsilon)} \leq 2 \delta_j \sqrt{n} \right\}\right) \leq \frac 1{3 \gamma_{j+1}}
	\end{align}
	But we have already seen that
	\begin{align}
		\mu_{j + 1}(A_{j+1}'(f, \epsilon)) \geq \frac 2{3 \gamma_{j+1}}
	\end{align}
	and as noted, for any $\vbf' \in A_{j+1}'(f,\epsilon)$, $\norm{\vbf_{f,j}(\epsilon) - \vbf'(\epsilon)} \leq 2 \delta_j \sqrt n$.  Thus $\mu_{j + 1}$ takes measure at least $\frac 1{3 \gamma_{j+1}}$ on the set of such desirable next links in the chain and so such a $\vbf_{f,j+1}$ exists.  Thus for any $f$, on this $\epsilon$, we have a chain $\vbf_{f,j}$ for $j \geq j_0$ such that $\vbf_{f, j} \in A_j'(f, \epsilon)$.  Note that, by \eqref{eq:triangle} and the way we have constructed the chain, we have that for all $f$,
	\begin{equation}
		\abs{\mathbb{T}_{\vbf_{f,j}, \vbf_{f,j+1}}(\epsilon)} \leq  C \sqrt n \norm{\vbf_{f,j}(\epsilon) - \vbf_{f,j+1}(\epsilon)} \sqrt{\log \gamma_j} \leq C \sqrt n \delta_j 2^{\frac j2}
	\end{equation}
	We also have for any $f$ that
	\begin{equation}
		\abs{\mathbb{T}_{\vbf_{f,j_0}}} \leq C  \sqrt{n \log \frac 1\rho}
	\end{equation}
	Thus we see that on this $\epsilon$,
	\begin{align}
		\sup_{f \in \mathcal{F}} \mathbb{T}_f(\epsilon) &= \sup_{f \in \mathcal{F}} \left(\mathbb{T}_{\vbf_{f,j_0}(\epsilon)} + \sum_{N \geq j \geq j_0} \mathbb{T}_{\vbf_{f,j+1}}(\epsilon) - \mathbb{T}_{\vbf_{f,j}}(\epsilon) + \mathbb{T}_{f(\z), \vbf_{f,N}}(\epsilon) \right) \\
		&\leq \sup_{f \in \mathcal{F}}\mathbb{T}_{\vbf_{f,j_0}(\epsilon)} + \sup_{f \in \F} \mathbb{T}_{f(\z), \vbf_{f,N}}(\epsilon) +  \sum_{N \geq j \geq j_0} \sup_{f \in \mathcal{F}} \mathbb{T}_{\vbf_{f,j+1},\vbf_{f,j}}(\epsilon) \\
		&\leq C \sqrt{n \log \frac 1\rho} + \sup_{f \in \F} \mathbb{T}_{f(\z), \vbf_{f,N}}(\epsilon) + \sum_{j \geq j_0} C \sqrt n \delta_j 2^{\frac j2} \\
		&\leq C \sqrt{n \log \frac 1\rho} + C \delta_N n + \sum_{N \geq j \geq j_0} C \sqrt n \delta_j 2^{\frac j2}
	\end{align}
	where the last inequality follows from Cauchy-schwarz and the fact that $\vbf_{f,N} \in A_N(f, \epsilon)$.  As \hyperlink{events}{($\ast$)} occurs with probability at least $1 - \rho$, we have with the same probability that the above is bounded.  This concludes the proof, modulo Lemma \ref{lem:chainingunionbound}.
\end{proof}
All that remains is to prove Lemma \ref{lem:chainingunionbound}.  We introduce an auxiliary lemma for that purpose:
\begin{lemma}\label{lem:fubini}
	Let $\mu$ a measure on $\mathcal{V}$ and consider indicator variables $U(v, \epsilon)$.  Suppose that for each $v \in \supp \mu$, $\ee_\epsilon(U(v, \epsilon)) \leq \alpha \rho$.  Then with probability at least $1 - \rho$ on the $\epsilon$,
	\begin{equation}
		\ee_\mu\left(U(v,\epsilon)\right) \leq \alpha
	\end{equation}
\end{lemma}
\begin{proof}
	This follows immediately from Fubini's theorem and Markov's inequality.
\end{proof}
Using Lemma \ref{lem:fubini}, we are able to conclude the proof with:
\begin{lemma}\label{lem:chainingunionbound}
	Let $j_0 = \lceil\log\log \frac 1\rho \rceil$.  Then with probability at least $1 - \rho$, the following events hold:
	\begin{align}
		&\mu_{j_0}\left(\left\{\vbf | \abs{\mathbb{T}_\vbf(\epsilon)} > C \sqrt{n \log \frac 1\rho} \right\}\right) \leq \frac 1{3 \gamma_{j_0}}  \\
		&\forall j \geq j_0, \, \nu_j\left(\left\{(\vbf,\vbf') | \abs{\mathbb{T}_{\vbf,\vbf'}(\epsilon)} > C  \delta_j \sqrt{n \log \gamma_j} \text{ and } \norm{\vbf(\epsilon) - \vbf'(\epsilon)} \leq 2 \delta_j\sqrt{n} \right\}\right) \leq \frac{1}{9 \gamma_j \gamma_{j+1}}
	\end{align}
\end{lemma}
\begin{proof}
	Let $j_0 \geq \log\log \frac 1\rho$.  Then by Lemma \ref{lem:adaptivetail} with $y = n$, we have for any fixed $\vbf$,
	\begin{equation}
		\pp_\epsilon\left(\left\{\abs{\mathbb{T}_\vbf(\epsilon)} > C \sqrt{n \log \frac {6 \gamma_{j_0}}{ \rho}} \text{ and } \norm{\vbf(\epsilon)}^2 \leq n\right\}\right) \leq \frac 1{6 \gamma_{j_0} \rho}
	\end{equation}
	By $\abs{\vbf_t(\epsilon)} \leq 1$, however, we have
	\begin{equation}
		\pp_\epsilon\left(\left\{\abs{\mathbb{T}_\vbf(\epsilon)} > C \sqrt{n \log \frac {6 \gamma_{j_0}}{ \rho}} \right\}\right) = \pp_\epsilon\left(\left\{\abs{\mathbb{T}_\vbf(\epsilon)} > C \sqrt{n \log \frac {6 \gamma_{j_0}}{ \rho}} \text{ and } \norm{\vbf(\epsilon)}^2 \leq n\right\}\right)
	\end{equation}
	Note that
	\begin{equation}
		\log \frac{6 \gamma_{j_0}}{ \rho} = \log \frac 1\rho + \log 6 \gamma_{j_0} \leq C \log \frac 1\rho
	\end{equation}
	by the assumption on $j_0$ and the fact that $\gamma_{j_0} = 2^{2^{j_0}}$.  Thus by Lemma \ref{lem:fubini}, we have with probability at least $1 - \frac \rho 2$,
	\begin{align}
		\mu_{j_0}\left(\left\{\vbf | \abs{\mathbb{T}_\vbf(\epsilon)} > C \sqrt{n\log \frac 1\rho} \right\}\right) &\leq \frac 1{3 \gamma_{j_0}}
	\end{align}
	Now, recall that $\nu_j = \mu_j \otimes \mu_{j +1}$ and let $j \geq j_0$.  Again by Lemma \ref{lem:adaptivetail}, this time with $y = 4 \delta_j^2  n$, we have that  for any fixed $\vbf,\vbf'$,
	\begin{equation}
		\pp_\epsilon\left(\left\{\abs{\mathbb{T}_{\vbf,\vbf'}(\epsilon)} > C  \sqrt{4 \delta_j^2 n \log \frac{9\gamma_j \gamma_{j+1}}{2^{-j-3}\rho}} \text{ and } \norm{\vbf(\epsilon) - \vbf'(\epsilon)}^2 \leq 4 \delta_j^2 n \right\}\right)  \leq \frac{1}{9\gamma_j \gamma_{j+1} 2^{-j-3} \rho}
	\end{equation}
	Now, note that by $j \geq j_0$ and the definition of $\gamma_j$, we have
	\begin{align}
		\log \frac{9\gamma_j \gamma_{j+1}}{2^{-j-3}\rho} = \log 9 + 2^j + 2^{j+1} + j + 3 + \log \frac 1\rho \leq C 2^j = C \log \gamma_j
	\end{align}
	Thus by Lemma \ref{lem:fubini}, we have with probability at least $1 - 2^{-j-3} \rho$,
	\begin{align}
		\nu_j\left(\left\{(\vbf,\vbf') | \abs{\mathbb{T}_{\vbf,\vbf'}(\epsilon)} > C \delta_j \sqrt{n \log \gamma_j} \text{ and } \norm{\vbf(\epsilon) - \vbf'(\epsilon)} \leq 2 \delta_j \sqrt n \right\}\right) \leq \frac 1{9\gamma_j \gamma_{j+1}}
	\end{align}
	By a union bound, then, we see that the two events in the statement of the lemma hold with probability at least $1 - \rho$, as desired.
\end{proof}


==> Sections/proof-majorizing.tex <==
\section{Proof of Proposition \ref{prop:majorizingchain}}\label{app:majorizingchain}

Our proof proceeds very similarly to the proof of Theorem \ref{thm:chaining} presented in Appendix \ref{app:chaining}.  The primary difference is that instead of using Lemma \ref{lem:adaptivetail}, we need stronger control over $\T_\vbf$, that does not make an assumption on $\norm{\vbf(\epsilon)}$.  In passing to this stronger concentration bound, we lose a factor polynomial in $\log\log n$.  Adapted to our setting from \cite{bartlett2008high}, we recall
\begin{lemma}[\cite{bartlett2008high}]\label{lem:rakhlintail}
  Suppose that $\vbf$ is a binary tree of depth $n$ with values in $[0,1]$.  Then with probability at least $1 - \rho$,
  \begin{equation}
      \abs{\T_\vbf(\epsilon)} \leq \max\lp 2 \log\lp \frac{\log n}{\rho}\rp, 4 \norm{\vbf(\epsilon)} \sqrt{\log\lp\frac{\log n}{\rho}\rp}   \rp
  \end{equation}
\end{lemma}
Now we proceed as before, but let our scales $\delta_j$ depend on $f,\epsilon$.
\begin{proof}[Proof of \ref{prop:majorizingchain}]
  The second statment follows by integrating the tail bound provided by the first statement.  Similarly to the proof of \ref{thm:chaining}, it suffices to show that for any $\mu$ with high probability on $\epsilon$, uniformly for $f \in \F$,
  \begin{align}
      \T_f(\epsilon) &\leq C \sqrt{n \log \frac 1\rho} + \sqrt{n} \delta_N(f,\epsilon) + C \sum_{j = 0}^N \delta_j(f, \epsilon) \sqrt{\log \frac 1{\mu(B_\delta(f, \epsilon)}} \\
      &\leq C  \sqrt{n \log \frac 1\rho} + \sqrt{n} \delta_N(f,\epsilon) + C\sum_{j = 0}^N \delta_j(f, \epsilon) 2^{\frac j2}
  \end{align}
  where $\delta_j(f, \epsilon)$ is the minimal $\delta > 0$ such that $\mu(B_\delta(f, \epsilon)) \geq 2^{- 2^j} = \gamma_j^{-1}$.  As before, we need an analogue of Lemma \ref{lem:chainingunionbound}.  We claim that for $j_0 = \lceil \log\log \frac 1\rho\rceil$, then with probability at least $1 - \rho$, the following, which we refer to as \hypertarget{majorizingtarget}{$(\dagger)$}, holds.  Simultaeneously, for all $j \geq j_0$ such that
  \begin{equation}
      \delta_j(f, \epsilon) > \sqrt{\frac{\log\log n + \log \frac 1 \rho}{n}}
  \end{equation}
  the inequalities below hold
  \begin{align}
      &\mu\lp\left\{\vbf | \abs{\T_\vbf(\epsilon)} > C \sqrt{n \log \frac 1 \rho}\right\}\rp \leq \frac 1{4 \gamma_{j_0}} \\
      &\nu\lp\left\{ \abs{\T_{\vbf,\vbf'}(\epsilon)} > C \delta_j(f, \epsilon) \sqrt{n \log \lp \gamma_j \log n \rp } \text{ and } \norm{\vbf(\epsilon) - \vbf(\epsilon')} \leq 2 \delta_j(f, \epsilon) \sqrt n \right\} \rp \\
      &\leq \frac 1{9 \gamma_j \gamma_{j+1}}
  \end{align}
  where $\nu = \mu \otimes \mu$.  The proof of \hyperlink{majorizingtarget}{$(\dagger)$} is Lemma \ref{lem:majorizingtarget}; for now we suppose that the result holds.  Once again, we consider the sets
  \begin{align}
      A_j(f, \epsilon) &= \left\{\vbf| \norm{\vbf(\epsilon) - f(\z(\epsilon))} \leq \sqrt n \delta_j(f, \epsilon)\right\} \\
      A_j'(f, \epsilon) &= \\
      \left\{\vbf \in A_j(f,\epsilon)| \mu\lp\left\{\vbf' | &\abs{\T_{\vbf, \vbf'}} > C \delta_j(f,\epsilon)\sqrt{n \log\lp\gamma_j\logn\rp} \text{ and } \norm{\vbf(\epsilon) - \vbf'(\epsilon)} \leq 2 \delta_j(f,\epsilon) \sqrt{n}\right\}\rp \leq \frac 1{3 \gamma_{j+1}}\right\}
  \end{align}
  By construction, $\mu(A_j(f, \epsilon) \geq \frac 1{\gamma_j}$.  The lower bound on $\mu(A_j'(f, \epsilon))$ under the event \hyperlink{majorizingtarget}{$(\dagger)$} is proven in exactly the same manner as in Appendix \ref{app:chaining} and so we do not reprove the result.  Similarly, the construction of the chain of $\vbf_{f,j,\epsilon}$ such that
  \begin{equation}
    \abs{\T_{\vbf_{f,j,\epsilon}, \vbf_{f,j+1,\epsilon}}} \leq C \sqrt{n \log\log n} \delta_j(f, \epsilon) 2^{\frac j2}
  \end{equation}
  on \hyperlink{majorizingtarget}{$(\dagger)$} holds exactly as before.  Thus, on this $\epsilon$, for every $f$, we have
  \begin{align}
      \T_f(\epsilon) &= \T_{\vbf_{f,j_0,\epsilon}}(\epsilon) + \sum_{N \geq j \geq j_0} \T_{\vbf_{f, j, \epsilon},\vbf_{f,j+1,\epsilon}}(\epsilon) + \T_{f(\z), \vbf_{f,N,\epsilon}}(\epsilon) \\
      &\leq C \sqrt{n \log \frac 1 \rho} + C \delta_N(f, \epsilon) n + \sum_{N \geq j \geq j_0} C \sqrt{n \log\log n} \delta_j(f,\epsilon) 2^{\frac j2} \\
      &\leq C \sqrt{n \log \frac 1 \rho} + C \sqrt{n \log \lp \frac{\log n}{\rho}\rp} + \sqrt{n \log\log n}\int_{\sqrt{\frac{log \lp \frac{\log n}{\rho}\rp}{n}}}^1 \sqrt{\log \frac 1{\mu(B_\delta(f, \epsilon)}} d \delta
  \end{align}
  Where we let $\delta_N(f, \epsilon)$ the minimal $\delta$ such that
  \begin{align}
      \delta_N(f, \epsilon) > \sqrt{\frac{\log \log n + \log \frac 1\rho}{n}}
  \end{align}
  Taking the supremum over $f, \epsilon$ on the right hand side above, and then taking the infimum over $\mu$ yields the desired result.
\end{proof}
All that remains is to prove taht \hyperlink{majorizingtarget}{$(\dagger)$} holds:
\begin{lemma}\label{lem:majorizingtarget}
  Let $j_0$ be as above.  With probability at least $1 - \rho$ over $\epsilon$, we have both
  \begin{equation}
      &\mu\lp\left\{\vbf | \abs{\T_\vbf(\epsilon)} > C \sqrt{n \log \frac 1 \rho}\right\}\rp \leq \frac 1{4 \gamma_{j_0}}
  \end{equation}
  and for all $j \geq j_0$ such that
  \begin{equation}
      \delta_j(f, \epsilon) > \sqrt{\frac{\log\log n + \log \frac 1 \rho}{n}}
  \end{equation}
  we have
  \begin{align}
      &\nu\lp\left\{ \abs{\T_{\vbf,\vbf'}(\epsilon)} > C \delta_j(f, \epsilon) \sqrt{n \log \lp \gamma_j \log n \rp } \text{ and } \norm{\vbf(\epsilon) - \vbf(\epsilon')} \leq 2 \delta_j(f, \epsilon) \sqrt n \right\} \rp \\
      &\leq \frac 1{9 \gamma_j \gamma_{j+1}}
  \end{align}
\end{lemma}
\begin{proof}
\adamcomment{Include proof}
The probability of the first event is bounded in the same way as in Lemma \ref{lem:chainingunionbound}.  As long as
\begin{equation}
    \delta_j > \frac 12 \sqrt{\frac{\log\log n + \log \frac 1\rho}{n}}
\end{equation}
we may apply Lemma \ref{lem:majorizingtarget} to Lemma \ref{lem:fubini} in the same way that we applied Lemma \ref{lem:adaptivetail} in the proof of Lemma \ref{lem:chainingunionbound}.  The result follows.  \adamcomment{Should I rewrite all of this in a more detailed way or is this sufficient?}
\end{proof}


